Local Convergence Properties of SAGA/Prox-SVRG and Acceleration

Over the past ten years, driven by large scale optimisation problems arising from machine learning, the development of stochastic optimisation methods have witnessed a tremendous growth. However, despite their popularity, the theoretical understandings of these methods are quite limited in contrast to the deterministic optimisation methods. In this paper, we present a local convergence analysis for a typical type of stochastic optimisation methods: proximal variance reduced stochastic gradient methods, and mainly focus on the SAGA [12] and Prox-SVRG [43] algorithms. Under the assumption that the non-smooth component of the optimisation problem is partly smooth relative to a smooth manifold, we present a unified framework for the local convergence analysis of the SAGA/Prox-SVRG algorithms: (i) the sequences generated by the SAGA/Prox-SVRG are able to identify the smooth manifold in a finite number of iterations; (ii) then the sequence enters a local linear convergence regime. Beyond local convergence analysis, we also discuss various possibilities for accelerating these algorithms, including adapting to better local parameters, and applying higher-order deterministic/stochastic optimisation methods which can achieve super-linear convergence. Concrete examples arising from machine learning are considered to verify the obtained results.

==> tex/sec-preliminary.tex <==
\section{Preliminary materials}\label{sec:preliminary}



Throughout the paper, $\bbN$ denotes the set of non-negative integers and $k \in \bbN$ denotes the index. 
$\bbR^n$ is the Euclidean space of $n$ dimension, and $\Id$ denotes the identity operator on $\bbR^n$. For a nonempty convex set $\Omega \subset \bbR^n$, $\ri(\Omega)$ and $\rbd(\Omega)$ denote its relative interior and boundary respectively, $\Aff(\Omega)$ is its affine hull, and $\LinHull(\Omega) \eqdef \bbR(\Omega-\Omega)$ is the subspace parallel to it. 
% Denote $\iota_{\Omega}$ the indicator function of $\Omega$, $\sigma_\Omega$ its support function and $\proj_{\Omega}$ the orthogonal projector onto $\Omega$. % For a matrix $M$, $\ker(M)$ is its null-space.
% 
Denote $\proj_{\Omega}$ the orthogonal projector onto $\Omega$. 
Given a linear operator $L : \bbR^{m}  \to \bbR^{n}$, denote $L_T \eqdef L \circ \proj_T$. %, and $L^{+}$ its Moore-Penrose pseudo-inverse.
% 

Given a proper, convex and lower semi-continuous function $R$, the sub-differential is defined by $\partial R(x) \eqdef \Ba{ g\in\bbR^{n} | R(y) \geq R(x) + \iprod{g}{y-x} ,~ \forall y\in\bbR^{n} }$. 
% \beq\label{eq:partial-R}
% \partial R :  \bbR^n \setvalued \bbR^n ,~ x\mapsto \Ba{ g\in\bbR^{n} | R(y) \geq R(x) + \iprod{g}{y-x} ,~ \forall y\in\bbR^{n} } .
% \eeq
We say function $R$ is $\mu$-strongly convex for some $\mu > 0$ if $R(x) - \frac{\mu}{2} \norm{x}^2$ still is convex. 


\jingwei{define $\ell_{2}$-norm and possibly others}

\paragraph{Partial smoothness}

The fundamental tool of our analysis in this paper is \emph{partial smoothness} which was first proposed in \cite{Lewis-PartlySmooth}. 
% 
Let $\calM$ be a $C^2$-smooth embedded submanifold of $\bbR^n$ around a point $x$. To lighten the notation, henceforth we shall state $C^2$-manifold instead of $C^2$-smooth embedded submanifold of $\bbR^n$. The natural embedding of a submanifold $\calM$ into $\bbR^n$ permits to define a Riemannian structure on $\calM$, and we simply say $\calM$ is a Riemannian manifold. $\tanSp{\calM}{x}$ denotes the tangent space to $\calM$ at any point near $x$ in $\calM$. % More materials on manifolds are given in Section~\ref{subsec:riemgeom}.

% We are now ready to state formally the class of partly smooth functions through its regularity properties.


 \begin{definition}[Partly smooth function]\label{dfn:psf}
 Let $R \in \lsc(\bbR^n)$,
 $R$ is said to be \emph{partly smooth at $x$ relative to a set $\calM$} containing $x$ if $\partial R(x) \neq \emptyset$, and moreover
 \begin{description}[leftmargin=3cm]%[label={\rm (\roman{*})}]
 \item[{\textbf{Smoothness:}}] \label{PS:C2} 
 $\calM$ is a $C^2$-manifold around $x$, $R$ restricted to $\calM$ is $C^2$ around $x$.
 \item[{\textbf{Sharpness:}}] \label{PS:Sharp} 
 The tangent space $\tanSp{\calM}{x}$ coincides with $T_{x} \eqdef \LinHull\Pa{\partial R(x)}^\perp$.
 % (Sharpness) The tangent space $\tanSp{\calM}{x} =  \LinHull\Pa{\partial R(x)}^\bot$;
 \item[{\textbf{Continuity:}}] \label{PS:DiffCont} 
 The set-valued mapping $\partial R$ is continuous at $x$ relative to $\calM$.
 \end{description}
 \end{definition}


The class of partly smooth functions at $x$ relative to $\calM$ is denoted as $\PSF{x}{\calM}$. 
%
% One can easily show that a function in $\lsc(\bbR^n)$ which is locally polyhedral around $x$ is partly smooth at $x$ relative to $x+T_x$.
% {Polyhedrality also implies that the subdifferential is locally constant around $x$ along $x+T_x$.}
% Capitalizing on the results of \cite{Lewis-PartlySmooth}, it can be shown that under mild transversality conditions, the set of proper lsc convex and partly smooth functions is closed under addition and pre-composition by a linear operator. Moreover, absolutely permutation-invariant convex and partly smooth functions of the singular values of a real matrix, \ie spectral functions, are convex and partly smooth spectral functions of the matrix \cite{Daniilidis-SpectralIdent}. 
Many widely used non-smooth penalty functions in the literature are partly, such as sparsity promoting $\ell_{1}$-norm, group sparsity promoting $\ell_{1,2}$-norm, low rank promoting nuclear norm, etc; we refer to \cite{liang2016multi,liang2017activity} and the references therein for more examples of partly smooth function in both convex and non-convex scenarios. 
%

Below we present two properties of partly smooth functions. The first one is local normal sharpness which is obtained from \cite[Proposition~2.10]{Lewis-PartlySmooth}.

\begin{lemma}[Local normal sharpness]
\label{fact:sharp}
If $R \in \PSF{x}{\calM}$, then all $x' \in \calM$ near $x$ satisfy $\tanSp{\calM}{x'} = T_{x'}$. In particular, when $\calM$ is affine or linear, then
$T_{x'} = T_{x}$.
\end{lemma}



Next we provide expressions of the Riemannian gradient and Hessian (see Section~\ref{subsec:riemgeom} for definitions) for the case of partly smooth functions relative to a $C^2$-smooth submanifold. This is summarized in the following proposition which follows by combining \eqref{eq:RieGradient}, \eqref{eq:RieHessian}, Definition~\ref{dfn:psf}, Lemma~\ref{fact:sharp} and \cite[Proposition~17]{Daniilidis06} (or \cite[Lemma~2.4]{miller2005newton}).


\begin{proposition}[Riemannian gradient and Hessian]
\label{fact:gradhess}
If $R \in \PSF{x}{\calM}$, then for any $x' \in \calM$ near $x$
\[
\nabla_{\calM} R(x') = \proj_{T_{x'}}\pa{\partial R(x')} .
\]
For all $h \in T_{x'}$,
\[
\nabla^2_{\calM} R(x')h = \proj_{T_{x'}} \nabla^2 \widetilde{R}(x')h + \Wgtmap{x'}\Pa{h, \proj_{T_{x'}^\perp}\nabla \widetilde{R}(x')}  ,
\]
where $\widetilde{R}$ is a smooth representation of $R$ on $\calM$, and $\Wgtmap{x}\pa{\cdot, \cdot}: T_x \times T_x^\perp \to T_x$ is the Weingarten map of $\calM$ at $x$ (see Section~\ref{subsec:riemgeom} for definitions).
\end{proposition}


